Fractional Conformal Map, Qubit Dynamics and the Leggett-Garg Inequality

Any pure state of a qubit can be geometrically represented as a point on the extended complex plane through stereographic projection. By employing successive conformal maps on the extended complex plane, we can generate an effective discrete-time evolution of the pure states of the qubit. This work focuses on a subset of analytic maps known as fractional linear conformal maps. We show that these maps serve as a unifying framework for a diverse range of quantum-inspired conceivable dynamics, including (i) unitary dynamics,(ii) non-unitary but linear dynamics and (iii) non-unitary and non-linear dynamics where linearity (non-linearity) refers to the action of the discrete time evolution operator on the Hilbert space. We provide a characterization of these maps in terms of Leggett-Garg Inequality complemented with No-signaling in Time (NSIT) and Arrow of Time (AoT) conditions.

==> bibfile.tex <==


@CONTROL{REVTEX41Control}
@CONTROL{apsrev41Control,author="08",editor="1",pages="0",title="",year="1"}

@article{Manzano2020,
  doi = {10.1063/1.5115323},
  url = {https://doi.org/10.1063/1.5115323},
  year = {2020},
  month = feb,
  publisher = {{AIP} Publishing},
  volume = {10},
  number = {2},
  pages = {025106},
  author = {Daniel Manzano},
  title = {A short introduction to the Lindblad master equation},
  journal = {{AIP} Advances}
}

@article{Choi,
    author = {M-D Choi},
    title = {Completely Positive Linear Maps on Complex Matrices},
    journal = {Lin. Alg.
Appl. 10, 285–290} ,
    year = {1975}
}

@article{AKPan,
    author =  {A. K. Pan},
    title = {},
    journal = {Phys. Rev. A 102, 032206 (2020)},
    year = {2020} 
}

@article{Clemente,
    author = { L. Clemente and J. Kofler},
    title = ,
    journal = {Phys. Rev. A 91, 062103 },
    year = {(2015)}
}

@article{Majidy,
    author = {S.-S. Majidy, H. Katiyar, G. Anikeeva, J. Halliwell, and R.
Laflamme},
    title = ,
    journal = {Phys. Rev. A 100, 042325 },
    year = {2019}
}

@article{Huffman,
    author = { E. Huffman and A. Mizel},
    title = ,
    journal = {Phys. Rev. A 95, 032131} ,
    year = {(2017)}
}
@article{Joarder2022,
  title = {Loophole-Free Interferometric Test of Macrorealism Using Heralded Single Photons},
  author = {Joarder, Kaushik and Saha, Debashis and Home, Dipankar and Sinha, Urbasi},
  journal = {PRX Quantum},
  volume = {3},
  issue = {1},
  pages = {010307},
  numpages = {29},
  year = {2022},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PRXQuantum.3.010307},
  url = {https://link.aps.org/doi/10.1103/PRXQuantum.3.010307}
}
@article{najarbashi,
    author = {Najarbashi, Seifi},
    title = {Relation Between Stereographic Projection
and Concurrence Measure in Bipartite Pure
States},
    journal = {DOI 10.1007/s10773-016-3071-2} ,
    year = {2016}
}


@article{Nakahara2008,
  title={Quantum Computing - From Linear Algebra to Physical Realizations},
  author={Mikio Nakahara and Tetsuo Ohmi},
  year={2008},
  url={https://api.semanticscholar.org/CorpusID:10812575}
}

@article{Francis1983,
  title={Complex variables
harmonic and analytic functions},
  author={ Francis J. Flanigan},
  year={1983}
}

@article{Elias2003,
  title={Complex variables},
  author={  E. M. Stein and R. Shakarchi},
  year={2003}
}

@article{Yau2016,
  title={Computational Conformal Geometry},
  author={Shing-Tung Yau and Xianfeng Gu},
  year={2016},
  url={https://api.semanticscholar.org/CorpusID:117563466}
}


@article{Nevanlinna,
    author = {R. Nevanlinna and V. Paatero.}, 
    title = {Introduction to complex analysis. Translated
from the German by T. Kovari and G. S. Goodman. Addison-Wesley Publish- ¨
ing Co., Reading, Mass.-London-Don Mills, Ont., 1969,},
    journal = ,
    year = 
}

@article{Ahlfors,
    author = {L. V. Ahlfors}, 
    title = {Complex Analysis. 1979. McGraw-Hill, Inc., Singapore.},
    journal = ,
    year = 
}

@article{Rudin,
    author = {W. Rudin. },
    title = {Real and complex analysis. Tata McGraw-Hill Education, 1987},
    journal = ,
    year = 
}
@article{PalaciosLaloy2010,
  doi = {10.1038/nphys1641},
  url = {https://doi.org/10.1038/nphys1641},
  year = {2010},
  month = apr,
  publisher = {Springer Science and Business Media {LLC}},
  volume = {6},
  number = {6},
  pages = {442--447},
  author = {Agustin Palacios-Laloy and Fran{\c{c}}ois Mallet and Fran{\c{c}}ois Nguyen and Patrice Bertet and Denis Vion and Daniel Esteve and Alexander N. Korotkov},
  title = {Experimental violation of a Bell's inequality in time with weak measurement},
  journal = {Nature Physics}
}

@article{Kofler2013,
  title = {Condition for macroscopic realism beyond the Leggett-Garg inequalities},
  author = {Kofler, Johannes and Brukner, \ifmmode \check{C}\else \v{C}\fi{}aslav},
  journal = {Phys. Rev. A},
  volume = {87},
  issue = {5},
  pages = {052115},
  numpages = {5},
  year = {2013},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.87.052115},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.87.052115}
}

@article{XiaoLiu2019,
  title = {Strict experimental test of macroscopic realism in a light-matter-interfaced system},
  author = {Liu, Xiao and Zhou, Zong-Quan and Han, Yong-Jian and Li, Zong-Feng and Hu, Jun and Yang, Tian-Shu and Li, Pei-Yun and Liu, Chao and Li, Xue and Ma, Yu and Liang, Peng-Jun and Li, Chuan-Feng and Guo, Guang-Can},
  journal = {Phys. Rev. A},
  volume = {100},
  issue = {3},
  pages = {032106},
  numpages = {8},
  year = {2019},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.100.032106},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.100.032106}
}
@article{KimLee,
    author = {Jae-weon Lee, Chang Ho Kim, Eok Kyun Lee, Jaewan Kim,
and Soonchil Lee},
    title = ,
    journal = {Quantum Information Processing, Vol. 1, Nos. 1/2, April 2002 (# 2002,}
    year = {2002}
}

@article{Gilyen,
    author = {Gilyén, A., Kiss, T. & Jex, I.},  
    title = {Exponential Sensitivity and its Cost in Quantum Physics},
    journal = {Sci Rep 6, 20076 (2016).},
    year = {https://doi.org/10.1038/srep20076}
}


@article{KissT,
  title = {Complex chaos in the conditional dynamics of qubits},
  author = {Kiss, T. and Jex, I. and Alber, G. and Vym\ifmmode \check{e}\else \v{e}\fi{}tal, S.},
  journal = {Phys. Rev. A},
  volume = {74},
  issue = {4},
  pages = {040301},
  numpages = {4},
  year = {2006},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.74.040301},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.74.040301}
}


@article{EmaryC,
    author = {C. Emary, N. Lambert, F. Nori},
    title = {Leggett–Garg inequalities},
    journal = {Rep. Prog. Phys. 77, 016001 },
    year = {(2014)}
}

@article{Kofler,
  title = {Conditions for Quantum Violation of Macroscopic Realism},
  author = {Kofler, Johannes and Brukner, \ifmmode \check{C}\else \v{C}\fi{}aslav},
  journal = {Phys. Rev. Lett.},
  volume = {101},
  issue = {9},
  pages = {090403},
  numpages = {4},
  year = {2008},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.101.090403},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.101.090403}
}

@article{Sayan,
    author = {Sayan Ghosh, Anant V varma, Sourin Das},
    title = {Leggett–Garg inequality in Markovian quantum
dynamics: role of temporal sequencing of coupling
to bath
},
    journal = {J. Phys. A: Math. Theor. 56 205302},
    year = 2023
}
@article{Knee2016,
  doi = {10.1038/ncomms13253},
  url = {https://doi.org/10.1038/ncomms13253},
  year = {2016},
  month = nov,
  publisher = {Springer Science and Business Media {LLC}},
  volume = {7},
  number = {1},
  author = {George C. Knee and Kosuke Kakuyanagi and Mao-Chuang Yeh and Yuichiro Matsuzaki and Hiraku Toida and Hiroshi Yamaguchi and Shiro Saito and Anthony J. Leggett and William J. Munro},
  title = {A strict experimental test of macroscopic realism in a superconducting flux qubit},
  journal = {Nature Communications}
}

@book{Bell1964, 
place={Cambridge et autres}, 
title={Speakable and unspeakable in quantum mechanics: Collected papers on quantum philosophy}, 
publisher={Cambridge Univ. Press}, author={Bell, 
John Steward and Aspect, Alain}, 
year={2013}
} 
@article{PLu2023,
      title={Experimental demonstration of enhanced violations of Leggett-Garg inequalities in a $\mathcal{PT}$-symmetric trapped-ion qubit}, 
      author={Pengfei Lu and Xinxin Rao and Teng Liu and Yang Liu and Ji Bian and Feng Zhu and Le Luo},
      year={2023},
      eprint={2309.06713},
      archivePrefix={arXiv},
      primaryClass={quant-ph}
}


@article{quinn2023,
      title={Observing super-quantum correlations across the exceptional point in a single, two-level trapped ion}, 
      author={Alexander Quinn and Jeremy Metzner and Jacob E. Muldoon and Isam Daniel Moore and Sean Brudney and Sourin Das and David T. C. Allcock and Yogesh N. Joglekar},
      year={2023},
      eprint={2304.12413},
      archivePrefix={arXiv},
      primaryClass={quant-ph}
}

@Article{Peres1999,
author={Peres, Asher},
title={All the Bell Inequalities},
journal={Foundations of Physics},
year={1999},
month={Apr},
day={01},
volume={29},
number={4},
pages={589-614},
abstract={Bell inequalities are derived for any number of observers, any number of alternative setups for each one of them and any number of distinct outcomes for each experiment. It is shown that if a physical system consists of several distant subsystems, and if the results of tests performed on the latter are determined by local variables with objective values, then the joint probabilities for triggering any given set of distant detectors are convex combinations of a finite number of Boolean arrays, whose components are either 0 or 1 according to a simple rule. This convexity property is both necessary and sufficient for the existence of local objective variables. It leads to a simple graphical method which produces a large number of generalized Clauser-Horne inequalities corresponding to the faces of a convex polytope. It is plausible that quantum systems whose density matrix has a positive partial transposition satisfy all these inequalities, and therefore are compatible with local objective variables, even if their quantum properties are essentially non-local.},
issn={1572-9516},
doi={10.1023/A:1018816310000},
url={https://doi.org/10.1023/A:1018816310000}
}


@article{Mahler1993,
  title = {Proposed test for temporal Bell inequalities},
  author = {Paz, Juan Pablo and Mahler, G\"unter},
  journal = {Phys. Rev. Lett.},
  volume = {71},
  issue = {20},
  pages = {3235--3239},
  numpages = {0},
  year = {1993},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.71.3235},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.71.3235}
}


@article{Kim2006,
  title = {Generic Bell Inequalities for Multipartite Arbitrary Dimensional Systems},
  author = {Son, W. and Lee, Jinhyoung and Kim, M. S.},
  journal = {Phys. Rev. Lett.},
  volume = {96},
  issue = {6},
  pages = {060406},
  numpages = {4},
  year = {2006},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.96.060406},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.96.060406}
}

@article{Budroni2013,
  title = {Bounding Temporal Quantum Correlations},
  author = {Budroni, Costantino and Moroder, Tobias and Kleinmann, Matthias and G\"uhne, Otfried},
  journal = {Phys. Rev. Lett.},
  volume = {111},
  issue = {2},
  pages = {020403},
  numpages = {5},
  year = {2013},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.111.020403},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.111.020403}
}
@article{Yogesh,
    author = {A V. Varma, J E. Muldoon, Sourav Paul, Y N. Joglekar and S Das},
    title = {Extreme violation of the Leggett-Garg inequality in nonunitary dynamics with complex energies},
    journal = {PHYSICAL REVIEW A 108, 032202 (2023)},
    year = {2023}
}

@article{Zhan,
    author ={Tianxiang Zhan, Chunwang Wu, Manchao Zhang, Qingqing Qin, Xueying Yang, Han Hu, Wenbo Su, Jie Zhang, Ting Chen, Yi Xie, Wei Wu, and Pingxing Chen} ,
    title = {Experimental violation of the Leggett-Garg inequality in a three-level trapped-ion system},
    journal = {Phys. Rev. A 107 012424 (2023)},
    year = {2023}
}

@article{Lindblad,
    author = {G. Lindblad},
    title = {Completely Positive Maps and Entropy Inequalities},
    journal = {Math. Phys. 40, 147-151 },
    year = {1975}
}
@article{Tusun,
    author = {Maimaitiyiming Tusun, Wei Cheng, Zihua Chai, Yang Wu, Ya Wang, Xing Rong, and Jiangfeng Du} ,
    title = {Experimental violation of the Leggett-Garg inequality with a single-spin system},
    journal = {Phys. Rev. A 105, 042613},
    year = {2022}
}
@article{LG1985,
  title = {Quantum mechanics versus macroscopic realism: Is the flux there when nobody looks?},
  author = {Leggett, A. J. and Garg, Anupam},
  journal = {Phys. Rev. Lett.},
  volume = {54},
  issue = {9},
  pages = {857--860},
  numpages = {0},
  year = {1985},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.54.857},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.54.857}
}


@article{Leggett2008,
	doi = {10.1088/0034-4885/71/2/022001},
	url = {https://doi.org/10.1088/0034-4885/71/2/022001},
	year = 2008,
	month = {jan},
	publisher = {{IOP} Publishing},
	volume = {71},
	number = {2},
	pages = {022001},
	author = {A J Leggett},
	title = {Realism and the physical world},
	journal = {Reports on Progress in Physics},
	abstract = {I consider the extent to which the applicability of the concept of classical realism is constrained, irrespective of the validity or not of the quantum formalism, by existing experiments both in the EPR–Bell setup, including recent experiments testing ‘nonlocal realistic’ theories, and in the area of ‘macroscopic quantum coherence’. Unless we are willing to sacrifice one or more other intuitively plausible notions such as that of the conventional ‘arrow of time’, it appears impossible, in either context, to maintain the classical notion of realism.}
}

@article{Leggett2002,
	doi = {10.1088/0953-8984/14/15/201},
	url = {https://doi.org/10.1088/0953-8984/14/15/201},
	year = 2002,
	month = {apr},
	publisher = {{IOP} Publishing},
	volume = {14},
	number = {15},
	pages = {R415--R451},
	author = {A J Leggett},
	title = {Testing the limits of quantum mechanics: motivation, state of play, prospects},
	journal = {Journal of Physics: Condensed Matter},
	abstract = {I present the motivation for experiments which attempt to generate, and verify the existence of, quantum superpositions of two or more states which are by some reasonable criterion `macroscopically' distinct, and show that various a priori objections to this programme made in the literature are flawed. I review the extent to which such experiments currently exist in the areas of free-space molecular diffraction, magnetic biomolecules, quantum optics and Josephson devices, and sketch possible future lines of development of the programme.}
}


@article{LGIreview2014,
	doi = {10.1088/0034-4885/77/1/016001},
	url = {https://doi.org/10.1088/0034-4885/77/1/016001},
	year = 2013,
	month = {dec},
	publisher = {{IOP} Publishing},
	volume = {77},
	number = {1},
	pages = {016001},
	author = {Clive Emary and Neill Lambert and Franco Nori},
	title = {Leggett{\textendash}Garg inequalities},
	journal = {Reports on Progress in Physics},
	abstract = {In contrast to the spatial Bell's inequalities which probe entanglement between spatially separated systems, the Leggett–Garg inequalities test the correlations of a single system measured at different times. Violation of a genuine Leggett–Garg test implies either the absence of a realistic description of the system or the impossibility of measuring the system without disturbing it. Quantum mechanics violates the inequalities on both accounts and the original motivation for these inequalities was as a test for quantum coherence in macroscopic systems. The last few years has seen a number of experimental tests and violations of these inequalities in a variety of microscopic systems such as superconducting qubits, nuclear spins, and photons. In this article, we provide an introduction to the Leggett–Garg inequalities and review these latest experimental developments. We discuss important topics such as the significance of the non-invasive measurability assumption, the clumsiness loophole, and the role of weak measurements. Also covered are some recent theoretical proposals for the application of Leggett–Garg inequalities in quantum transport, quantum biology and nano-mechanical systems.}
}


@Article{Wilde2012,
author={Wilde, Mark M.
and Mizel, Ari},
title={Addressing the Clumsiness Loophole in a Leggett-Garg Test of Macrorealism},
journal={Foundations of Physics},
year={2012},
month={Feb},
day={01},
volume={42},
number={2},
pages={256-265},
abstract={The rise of quantum information theory has lent new relevance to experimental tests for non-classicality, particularly in controversial cases such as adiabatic quantum computing superconducting circuits. The Leggett-Garg inequality is a ``Bell inequality in time'' designed to indicate whether a single quantum system behaves in a macrorealistic fashion. Unfortunately, a violation of the inequality can only show that the system is either (i) non-macrorealistic or (ii) macrorealistic but subjected to a measurement technique that happens to disturb the system. The ``clumsiness'' loophole (ii) provides reliable refuge for the stubborn macrorealist, who can invoke it to brand recent experimental and theoretical work on the Leggett-Garg test inconclusive. Here, we present a revised Leggett-Garg protocol that permits one to conclude that a system is either (i) non-macrorealistic or (ii) macrorealistic but with the property that two seemingly non-invasive measurements can somehow collude and strongly disturb the system. By providing an explicit check of the invasiveness of the measurements, the protocol replaces the clumsiness loophole with a significantly smaller ``collusion'' loophole.},
issn={1572-9516},
doi={10.1007/s10701-011-9598-4},
url={https://doi.org/10.1007/s10701-011-9598-4}
}



@article{Emary2014,
  title = {Temporal Quantum Correlations and Leggett-Garg Inequalities in Multilevel Systems},
  author = {Budroni, Costantino and Emary, Clive},
  journal = {Phys. Rev. Lett.},
  volume = {113},
  issue = {5},
  pages = {050401},
  numpages = {5},
  year = {2014},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.113.050401},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.113.050401}
}



@article{Fritz2010,
	doi = {10.1088/1367-2630/12/8/083055},
	url = {https://doi.org/10.1088/1367-2630/12/8/083055},
	year = 2010,
	month = {aug},
	publisher = {{IOP} Publishing},
	volume = {12},
	number = {8},
	pages = {083055},
	author = {Tobias Fritz},
	title = {Quantum correlations in the temporal Clauser{\textendash}Horne{\textendash}Shimony{\textendash}Holt ({CHSH}) scenario},
	journal = {New Journal of Physics},
	abstract = {We consider a temporal version of the Clauser–Horne–Shimony–Holt (CHSH) scenario using projective measurements on a single quantum system. It is known that quantum correlations in this scenario are fundamentally more general than correlations obtainable with the assumptions of macroscopic realism and non-invasive measurements. In this paper, we also educe some fundamental limitations of these quantum correlations. One result is that a set of correlators can appear in the temporal CHSH scenario if and only if it can appear in the usual spatial CHSH scenario. In particular, we derive the validity of the Tsirelson bound and the impossibility of Popescu–Rohrlich (PR)-box behavior. The strength of possible signaling also turns out to be surprisingly limited, giving a maximal communication capacity of approximately 0.32 bit. We also find a temporal version of Hardy's non-locality paradox with a maximal quantum value of 1/4.}
}

@article{Lindblad1976,
  doi = {10.1007/bf01608499},
  url = {https://doi.org/10.1007/bf01608499},
  year = {1976},
  month = jun,
  publisher = {Springer Science and Business Media {LLC}},
  volume = {48},
  number = {2},
  pages = {119--130},
  author = {G. Lindblad},
  title = {On the generators of quantum dynamical semigroups},
  journal = {Communications in Mathematical Physics}
}

@article{Gorini1976,
  doi = {10.1063/1.522979},
  url = {https://doi.org/10.1063/1.522979},
  year = {1976},
  publisher = {{AIP} Publishing},
  volume = {17},
  number = {5},
  pages = {821},
  author = {Vittorio Gorini and Andrzej Kossakowski and E. C. G. Sudarshan},
  title = {Completely positive dynamical semigroups of N-level systems},
  journal = {Journal of Mathematical Physics}
}

@article{plenio1,
  doi = {10.1103/physrevlett.113.140401},
  url = {https://doi.org/10.1103/physrevlett.113.140401},
  year = {2014},
  month = sep,
  publisher = {American Physical Society ({APS})},
  volume = {113},
  number = {14},
  author = {T.  Baumgratz and M.  Cramer and M.B.  Plenio},
  title = {Quantifying Coherence},
  journal = {Physical Review Letters}
}

@article{lock,
  doi = {10.1103/revmodphys.77.513},
  url = {https://doi.org/10.1103/revmodphys.77.513},
  year = {2005},
  month = jun,
  publisher = {American Physical Society ({APS})},
  volume = {77},
  number = {2},
  pages = {513--577},
  author = {Samuel L. Braunstein and Peter van Loock},
  title = {Quantum information with continuous variables},
  journal = {Reviews of Modern Physics}
}

@article{vendral,
  doi = {10.1103/revmodphys.84.1655},
  url = {https://doi.org/10.1103/revmodphys.84.1655},
  year = {2012},
  month = nov,
  publisher = {American Physical Society ({APS})},
  volume = {84},
  number = {4},
  pages = {1655--1707},
  author = {Kavan Modi and Aharon Brodutch and Hugo Cable and Tomasz Paterek and Vlatko Vedral},
  title = {The classical-quantum boundary for correlations: Discord and related measures},
  journal = {Reviews of Modern Physics}
}

@article{lupo,
  doi = {10.1103/revmodphys.86.1203},
  url = {https://doi.org/10.1103/revmodphys.86.1203},
  year = {2014},
  month = dec,
  publisher = {American Physical Society ({APS})},
  volume = {86},
  number = {4},
  pages = {1203--1259},
  author = {Filippo Caruso and Vittorio Giovannetti and Cosmo Lupo and Stefano Mancini},
  title = {Quantum channels and memory effects},
  journal = {Reviews of Modern Physics}
}

@article{lian,
  doi = {10.1103/physreva.91.042120},
  url = {https://doi.org/10.1103/physreva.91.042120},
  year = {2015},
  month = apr,
  publisher = {American Physical Society ({APS})},
  volume = {91},
  number = {4},
  author = {Lian-He Shao and Zhengjun Xi and Heng Fan and Yongming Li},
  title = {Fidelity and trace-norm distances for quantifying coherence},
  journal = {Physical Review A}
}

@misc{sayan,
  doi = {10.48550/ARXIV.2110.10696},
  url = {https://arxiv.org/abs/2110.10696},
  author = {Ghosh,  Sayan and Varma,  Anant V. and Das,  Sourin},
  keywords = {Quantum Physics (quant-ph),  Other Condensed Matter (cond-mat.other),  FOS: Physical sciences,  FOS: Physical sciences},
  title = {Leggett-Garg inequality in Markovian quantum dynamics: role of temporal sequencing of coupling to bath},
  publisher = {arXiv},
  year = {2021},
  copyright = {arXiv.org perpetual,  non-exclusive license}
}

@article{Anant,
  doi = {10.1088/1751-8121/abde76},
  url = {https://doi.org/10.1088/1751-8121/abde76},
  year = {2021},
  month = feb,
  publisher = {{IOP} Publishing},
  volume = {54},
  number = {11},
  pages = {115301},
  author = {Anant V Varma and Ipsika Mohanty and Sourin Das},
  title = {Temporal correlation beyond quantum bounds in non-Hermitian {PT}- symmetric dynamics of a two level system},
  journal = {Journal of Physics A: Mathematical and Theoretical}
}

@article{Usha,
  doi = {10.1103/physreva.103.032420},
  url = {https://doi.org/10.1103/physreva.103.032420},
  year = {2021},
  month = mar,
  publisher = {American Physical Society ({APS})},
  volume = {103},
  number = {3},
  author = {H. S. Karthik and H. Akshata Shenoy and A. R. Usha Devi},
  title = {Leggett-Garg inequalities and temporal correlations for a qubit under 
		$\less$mml:math xmlns:mml="http://www.w3.org/1998/Math/{MathML}"$\greater$$\less$mml:mi mathvariant="script"$\greater${PT}$\less$/mml:mi$\greater$$\less$/mml:math$\greater$
		-symmetric dynamics},
  journal = {Physical Review A}
}

@article{Anandan1990,
  doi = {10.1103/physrevlett.65.1697},
  url = {https://doi.org/10.1103/physrevlett.65.1697},
  year = {1990},
  month = oct,
  publisher = {American Physical Society ({APS})},
  volume = {65},
  number = {14},
  pages = {1697--1700},
  author = {J. Anandan and Y. Aharonov},
  title = {Geometry of quantum evolution},
  journal = {Physical Review Letters}
}

@article{Pan,
	doi = {10.1088/1751-8121/ac0546},
	url = {https://doi.org/10.1088/1751-8121/ac0546},
	year = 2021,
	month = {jun},
	publisher = {{IOP} Publishing},
	volume = {54},
	number = {27},
	pages = {275303},
	author = {Javid Naikoo and Swati Kumari and Subhashish Banerjee and A K Pan},
	title = {{PT}
			    
			   symmetric evolution, coherence and violation of Leggett{\textendash}Garg inequalities},
	journal = {Journal of Physics A: Mathematical and Theoretical},
	abstract = {We report an unusual buildup of the quantum coherence in a qubit subjected to non-Hermitian evolution generated by a parity-time () symmetric Hamiltonian, which is reinterpreted as a Hermitian system in a higher dimensional space using Naimark dilation. The coherence is found to be maximum about the exceptional points (EPs), i.e. the points of coalescence of the eigenvalues as well as the eigenvectors. The nontrivial physics about EPs has been observed in various systems, particularly in photonic systems. As a consequence of enhancement in coherence, the various formulations of Leggett–Garg inequality tests show maximal violation about the EPs.}
}


@article{Brody,
  title = {Mixed-State Evolution in the Presence of Gain and Loss},
  author = {Brody, Dorje C. and Graefe, Eva-Maria},
  journal = {Phys. Rev. Lett.},
  volume = {109},
  issue = {23},
  pages = {230405},
  numpages = {5},
  year = {2012},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.109.230405},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.109.230405}
}

@article{Alber1999,
author = {Alber, G.},
year = {1999},
month = {11},
pages = {},
title = {Entanglement And The Linearity Of Quantum Mechanics}
}

@article{David2022,
  title = {Follow the Math!:
The mathematics of quantum mechanics as the mathematics
of set partitions linearized to (Hilbert) vector spaces.
},
  author = {David Ellerman},
  numpages = {33},
  year = {2022},
  month = {July},
  url = {https://arxiv.org/pdf/2208.00384.pdf}}

@Article{Emilio2020,
AUTHOR = {Fiordilino, Emilio},
TITLE = {The Emergence of Chaos in Quantum Mechanics},
JOURNAL = {Symmetry},
VOLUME = {12},
YEAR = {2020},
NUMBER = {5},
ARTICLE-NUMBER = {785},
URL = {https://www.mdpi.com/2073-8994/12/5/785},
ISSN = {2073-8994},
ABSTRACT = {Nonlinearity in Quantum Mechanics may have extrinsic or intrinsic origins and is a liable route to a chaotic behaviour that can be of difficult observations. In this paper, we propose two forms of nonlinear Hamiltonian, which explicitly depend upon the phase of the wave function and produce chaotic behaviour. To speed up the slow manifestation of chaotic effects, a resonant laser field assisting the time evolution of the systems causes cumulative effects that might be revealed, at least in principle. The nonlinear Schr&ouml;dinger equation is solved within the two-state approximation; the solution displays features with characteristics similar to those found in chaotic Classical Mechanics: sensitivity on the initial state, dense power spectrum, irregular filling of the Poincar&eacute; map and exponential separation of the trajectories of the Bloch vector &sigma; in the Bloch sphere.},
DOI = {10.3390/sym12050785}
}


@article{Wm2006,
author = {Mcharris, Wm},
year = {2006},
month = {11},
pages = {},
title = {On the Possibility of Nonlinearities and Chaos Underlying Quantum Mechanics}
}

@article{Wright2021,
  title = {Automatic post-selection by ancillae thermalization},
  author = {Wright, L. and Barratt, F. and Dborin, J. and Booth, G. H. and Green, A. G.},
  journal = {Phys. Rev. Research},
  volume = {3},
  issue = {3},
  pages = {033151},
  numpages = {12},
  year = {2021},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevResearch.3.033151},
  url = {https://link.aps.org/doi/10.1103/PhysRevResearch.3.033151}
}


@article{Poincare,
author = {Poincare, H.},
year = {1892},
month = {},
pages = {},
title = {Les Méthodes Nouvelles de la Méchanique Céleste}
}


@article{Bountis1995,
  title = {Fundamental concepts of classical chaos I},
  author = {Bountis, Tassos},
  journal = {Open Systems & Information Dynamics},
  volume = {},
  issue = {},
  pages = {},
  numpages = {},
  year = {1995},
  month = {Aug},
  publisher = {},
  doi = {10.1007/BF02228810},
  url = {https://doi.org/10.1007/BF02228810}
}

@article{Julia,
author = {Julia, G.},
year = {1918},
month = {},
pages = {},
title = {Mémoire sur l'iteration des fonctions rationnelles}
}

@article{Fatou,
author = {Fatou, P.},
year = {1917},
month = {},
pages = {},
title = {Sur les substitutions rationnelles}
}


@article{Alber2001,
  title = {Efficient bipartite quantum state purification in arbitrary dimensional Hilbert spaces},
  author = {Alber G.,Delgado1 A., Gisin N. and Jex I.},
  journal = {Phys. A: Math. Gen, 34 8821 },
  volume = {},
  issue = {},
  pages = {},
  numpages = {},
  year = {2001},
  month = {Aug},
  publisher = {},
  doi = {10.1088/0305-4470/34/42/307},
  url = {https://doi.org/10.1088/0305-4470/34/42/307}
}
